Improved convergence of forward and inverse finite element models

Forward and inverse models are used throughout different engineering fields to predict and understand the behaviour of systems and to find parameters from a set of observations. These models use root-finding and minimisation techniques respectively to achieve their goals. This paper introduces improvements to these mathematical methods to then improve the convergence behaviour of the overarching models when used in highly non-linear systems. The performance of the new techniques is examined in detail and compared to that of the standard methods. The improved techniques are also tested with FEM models to show their practical application. Depending on the specific configuration of the problem, the improved models yielded larger convergence basins and/or took fewer steps to converge.

==> Chapters/Extended_Newton.tex <==
\subsubsection{Extended Formulation}
In the extended formulation the Jacobian becomes a rectangular matrix of size $[n^2\times n]$, where $n$ stands for the number of equations of the system or in other words the dimension of the system. This new Jacobian matrix will be referenced as the "extended Jacobian" from here on. The inverse of the extended Jacobian will be denoted by $p_{ij}$ which has the transpose shape of the extended Jacobian. The function vector $f_k(x_i^n)$ is extended to align with the shape of $p_{ij}$ to a $[n^2\times 1]$ column vector and is written as $q_j$. The vector $x_{i}^{n}$ remains unchanged. These changes can finally be written as:
\begin{equation} \label{eq:exn}
x_i^{n+1} = x_i^n - p_{ij}q_{j}
\end{equation}
Where $p_{ij}$ is the pseudo inverse of the extended Jacobian matrix and $q_{j}$ is the extended column vector of the original function vector.
\subsubsection{Jacobian assembly}
The Jacobian matrix of a vector function is the matrix of all partial first order derivatives. The extended Jacobian of the new modified iterable function $q_j$ is a rectangular matrix denoted by $b_{ji}$. It is calculated using the following:
\begin{equation}
    b_{ji} = \dfrac{\partial q_j}{\partial x_i}
\end{equation}
\subsubsection{Pseudo inverse of $b_{ji} \rightarrow p_{ij}$}
The pseudo inverse or otherwise known as a Moore–Penrose inverse is a generalisation of the inverse matrix denoted by $\bm{A^{+}}$. The matrix is commutable and has the transpose shape of the original maintaining a connection with the original terms. A pseudo inverse is a linear map between row and column space. It possess the following properties: \newline
\begin{equation}
\begin{array}{lcl}
    \bm{AA^{+}A} & = & \bm{A}\\
    \bm{AA^{+}A} & = & \bm{A}\\
    \bm{A^{+}AA^{+}} & = & \bm{A^{+}}
\end{array}
\end{equation}
The most popular way of calculating the pseudo inverse is to use Single Value Decomposition or SVD \cite{svdpseudo}.
Multiple software packages offer this feature. In this case NumPy's pinv() function was used. The resulting inverse matrix is denoted by $p_{ij}$.

==> figures/validation.tex <==
\begin{asy}
settings.render=0;
import graph3;
size(14cm,10cm);

currentprojection=perspective(1.5,-2,0.5);

xaxis3("$x$",0,4,grey,OutTicks(4,2));
yaxis3("$y$",-1,1,grey,OutTicks(1,-1));
zaxis3("$z$",-1,1,grey,OutTicks(1,-1));
//draw(O -- 4X, arrow=Arrow3, L=Label("$x$", position=EndPoint,
//align=W));
//draw(O -- 1.5Y, arrow=Arrow3, L=Label("$y$", position=EndPoint));
//draw(O -- 1.5Z, arrow=Arrow3, L=Label("$z$", position=EndPoint));

//real [] x = {0,0.4,0.8,1.2,1.6,2};
//real [] l = {1,2.05165229674338, 2.051651026534028, 2.051595887556811, 2.0514603140906673, 2.0514591428534046};
real [] l = {1,2.46644139, 2.43561483, 1.5502766,  1.23447845, 1.23322069};     
real [] l2 = {1,1.7840080477005023, 1.784007972898496, 1.7840058245862433, 1.7840050582880906, 1.7840050552360942};
real [] l1 = {1,1,1,1,1,1};
real [] y = {-0.5,0.5};
real [] z = {-0.5,0.5};
int end = 6;
real step = 0.4;
real x = -step;
for (int i=0; i<end;i+=1)
{
l1[i] = 1/sqrt(l[i]);
}
for (int i = 0; i<end; i+=1)
{
x +=step*l2[i];
draw(((x, y[0]*l1[i],z[0]*l1[i])--(x, y[1]*l1[i],z[0]*l1[i])--(x, y[1]*l1[i],z[1]*l1[i])--(x, y[0]*l1[i],z[1]*l1[i])--cycle));
if(i!=end-1)
{
draw((x, y[0]*l1[i],z[0]*l1[i])--(x+step*l2[i+1], y[0]*l1[i+1],z[0]*l1[i+1]));
draw((x, y[1]*l1[i],z[0]*l1[i])--(x+step*l2[i+1], y[1]*l1[i+1],z[0]*l1[i+1]));
draw((x, y[1]*l1[i],z[1]*l1[i])--(x+step*l2[i+1] ,y[1]*l1[i+1],z[1]*l1[i+1]));
draw((x, y[0]*l1[i],z[1]*l1[i])--(x+step*l2[i+1] ,y[0]*l1[i+1],z[1]*l1[i+1]));
}
}
\end{asy}
